Phase Separation, Capillarity, and Odd Surface Flows in Chiral Active Matter

Active phase separations evade canonical thermodynamic descriptions and have thus challenged our understanding of coexistence and interfacial phenomena. Considerable progress has been made towards a non-equilibrium theoretical description of these traditionally thermodynamic concepts. Spatial parity symmetry is conspicuously assumed in much of this progress, despite the ubiquity of chirality in experimentally realized systems. In this Letter, we derive a theory for the phase coexistence and interfacial fluctuations of a system which microscopically violates spatial parity. We find suppression of the phase separation as chirality is increased as well as the development of steady-state currents tangential to the interface dividing the phases. These odd flows are irrelevant to stationary interfacial properties, with stability, capillary fluctuations, and surface area minimization determined entirely by the capillary surface tension. Using large-scale Brownian dynamics simulations, we find excellent agreement with our theoretical scaling predictions.

==> custom-commands.tex <==
\usepackage{multirow}

% ******** CUSTOMIZATIONS  ******** %
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

%******** FONT FORMATTING ********%
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
%new command
\newcommand{\xmark}{\ding{55}}%
\newcommand*\diff{\mathop{}\!\mathrm{d}}

%When editing
%\newcommand{\ed}[1]{{\color{blue}#1}}
\newcommand{\ed}[1]{{\color{black}#1}}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}

\makeatletter
\DeclareRobustCommand{\svdots}{%
  \hbox{ }\vbox{%
    \baselineskip 3\p@
    \lineskiplimit \z@
    \kern 1\p@
    \hbox{.}\hbox{.}\hbox{.}%
  }%
  \hbox{ }
}
\makeatother

\makeatletter
\def\overvect@#1#2#3{\vbox{\ialign{##\crcr
       \noalign{\kern-.7pt\nointerlineskip}#1#2\crcr
       \noalign{\kern1pt\nointerlineskip}$\m@th\hfil#2#3\hfil$\crcr}}}
\makeatother
\def\*#1{\mathbf{#1}}
%\newcommand{\todo}[1]{\textcolor{RedViolet}{[ToDo: #1]}}
\newcommand{\fvect}[1]{\overset{\rightarrow}{#1}}
\newcommand{\bvect}[1]{\overset{\leftarrow}{#1}}
\newcommand{\scp}{\mathcal{P}}
\newcommand{\bscp}{\partial \scp}

\DeclareMathOperator\erfc{erfc}
% increase line spacing in matrix environments
\makeatletter
\renewcommand*\env@matrix[1][\arraystretch]{%
  \edef\arraystretch{#1}%
  \hskip -\arraycolsep
  \let\@ifnextchar\new@ifnextchar
  \array{*\c@MaxMatrixCols c}}
\makeatother

% better circled text
\newcommand*\circled[1]{
	\tikz[baseline=(char.base)]{
		\node[shape=circle,draw,inner sep=1pt] (char) {#1};
	}
}
%coloring in math mode
\makeatletter
\def\mathcolor#1#{\@mathcolor{#1}}
\def\@mathcolor#1#2#3{%
  \protect\leavevmode
  \begingroup
    \color#1{#2}#3%
  \endgroup
}
\makeatother

%short arrow that can rotate
\makeatletter
\newcommand{\fixed@sra}{$\vrule height 2\fontdimen22\textfont2 width 0pt\shortrightarrow$}
\newcommand{\shortarrow}[1]{%
  \mathrel{\text{\rotatebox[origin=c]{\numexpr#1*45}{\fixed@sra}}}
}
\makeatother
\makeatletter
\newcommand{\blankarrow}{\textcolor{white}{\shortarrow{1}}}
\makeatother

%boxing characters
\makeatletter
\renewcommand{\boxed}[1]{\text{\fboxsep=.2em\fbox{\m@th$\displaystyle#1$}}}
\makeatother

%small fraction
\newcommand\ddfrac[2]{\frac{\displaystyle #1}{\displaystyle #2}}
%\geometry{margin=1in}

%short to
\newcommand{\shortto}[1][3pt]{\mathrel{%
   \hbox{\rule[\dimexpr\fontdimen22\textfont2-.2pt\relax]{#1}{.4pt}}%
   \mkern-4mu\hbox{\usefont{U}{lasy}{m}{n}\symbol{41}}}}

\def\doubleunderline#1{\underline{\underline{#1}}}

%TikZ code "illustrating" the new "brace"
\newcommand{\newbrace}[1][]{
\begin{tikzpicture}[baseline=-0.5ex]
\draw[#1] (0,0) -- (0.3,0.3);
\draw[#1] (0,0) -- (0.3,-0.3);
\end{tikzpicture}
}

% the optional argument allows you to select the type of arrow 
% you can also customize the "new brace"
\newenvironment{casesnew}[1][->]%
{\;\newbrace[#1]\;\begin{array}{@{}l@{}}}%
{\end{array}}

%Declaring some math operators
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\sech}{sech}
\allowdisplaybreaks

\renewcommand{\thefigure}{S.\arabic{figure}}
\renewcommand{\thetable}{S.\arabic{table}}

\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\DontPrintSemicolon
% Define pseudocode formatting
\renewcommand{\KwSty}[1]{\textnormal{\textcolor{blue!90!black}{\ttfamily\bfseries #1}}\unskip}
\renewcommand{\ArgSty}[1]{\textnormal{\ttfamily #1}\unskip}
\SetKwComment{Comment}{\color{green!50!black}// }{}
\renewcommand{\CommentSty}[1]{\textnormal{\ttfamily\color{green!50!black}#1}\unskip}
\newcommand{\assign}{\leftarrow}
\newcommand{\var}{\texttt}
\newcommand{\FuncCall}[2]{\texttt{\bfseries #1(#2)}}
\SetKwProg{Function}{function}{}{}
\renewcommand{\ProgSty}[1]{\texttt{\bfseries #1}}


%%%%%%%%%%%%%%%%%%%%%%% Wide tilde %%%%%%%%%%%%
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{stackengine}
\usepackage{scalerel}

